Defending Against Image Corruptions Through Adversarial Augmentations

Modern neural networks excel at image classification, yet they remain vulnerable to common image corruptions such as blur, speckle noise or fog. Recent methods that focus on this problem, such as AugMix and DeepAugment, introduce defenses that operate in expectation over a distribution of image corruptions. In contrast, the literature on $\ell_p$-norm bounded perturbations focuses on defenses against worst-case corruptions. In this work, we reconcile both approaches by proposing AdversarialAugment, a technique which optimizes the parameters of image-to-image models to generate adversarially corrupted augmented images. We theoretically motivate our method and give sufficient conditions for the consistency of its idealized version as well as that of DeepAugment. Our classifiers improve upon the state-of-the-art on common image corruption benchmarks conducted in expectation on CIFAR-10-C and improve worst-case performance against $\ell_p$-norm bounded perturbations on both CIFAR-10 and ImageNet.

==> tables/mce_cifar.tex <==
\begin{center}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|ccc|cccc|cccc|cccc}
    \hline
    \cellcolor{header} & \cellcolor{header} & \multicolumn{3}{c|}{\cellcolor{header} \textsc{Noise}} & \multicolumn{4}{c|}{\cellcolor{header} \textsc{Blur}} & \multicolumn{4}{c|}{\cellcolor{header} \textsc{Weather}} & \multicolumn{4}{c}{\cellcolor{header} \textsc{Digital}} \Tstrut \\
    \cellcolor{header} \textsc{Setup} & \cellcolor{header} \textsc{mCE} & \cellcolor{header} \rotcol{Gauss} & \cellcolor{header} \rotcol{Shot} & \cellcolor{header} \rotcol{Impulse} & \cellcolor{header} \rotcol{Defocus} & \cellcolor{header} \rotcol{Glass} & \cellcolor{header} \rotcol{Motion} & \cellcolor{header} \rotcol{Zoom} & \cellcolor{header} \rotcol{Snow} & \cellcolor{header} \rotcol{Frost} &  \cellcolor{header} \rotcol{Fog} & \cellcolor{header} \rotcol{Bright} & \cellcolor{header} \rotcol{Contrast} & \cellcolor{header} \rotcol{Elastic} & \cellcolor{header} \rotcol{Pixel} & \cellcolor{header} \rotcol{JPEG} \Bstrut \\ \hline
\adaedsr  & 12.49\% & 25\showdecimals{8}\showpercentage & 19\showdecimals{8}\showpercentage & 29\showdecimals{9}\showpercentage & 9\showdecimals{3}\showpercentage & 15\showdecimals{6}\showpercentage & 10\showdecimals{9}\showpercentage & 9\showdecimals{6}\showpercentage & 9\showdecimals{3}\showpercentage & 8\showdecimals{1}\showpercentage & 8\showdecimals{8}\showpercentage & 4\showdecimals{3}\showpercentage & 11\showdecimals{0}\showpercentage & 9\showdecimals{3}\showpercentage & \textbf{6\showdecimals{7}\showpercentage} & 9\showdecimals{2}\showpercentage \Tstrut \\
\adaedsr + AugMix  & 8.80\% & 16\showdecimals{4}\showpercentage & 12\showdecimals{8}\showpercentage & 14\showdecimals{4}\showpercentage & 5\showdecimals{7}\showpercentage & 10\showdecimals{9}\showpercentage & 7\showdecimals{5}\showpercentage & 6\showdecimals{3}\showpercentage & \textbf{7\showdecimals{7}\showpercentage} & 6\showdecimals{7}\showpercentage & 6\showdecimals{6}\showpercentage & \textbf{3\showdecimals{9}\showpercentage} & \textbf{4\showdecimals{7}\showpercentage} & \textbf{8\showdecimals{1}\showpercentage} & 11\showdecimals{9}\showpercentage & 8\showdecimals{4}\showpercentage \\
\adaedsr + \DA + AugMix  & 8.58\% & 9\showdecimals{8}\showpercentage & 8\showdecimals{7}\showpercentage & 12\showdecimals{4}\showpercentage & 6\showdecimals{3}\showpercentage & 11\showdecimals{6}\showpercentage & 8\showdecimals{0}\showpercentage & 6\showdecimals{8}\showpercentage & 9\showdecimals{4}\showpercentage & 7\showdecimals{5}\showpercentage & 8\showdecimals{8}\showpercentage & 5\showdecimals{4}\showpercentage & 6\showdecimals{6}\showpercentage & 9\showdecimals{2}\showpercentage & 9\showdecimals{7}\showpercentage & 8\showdecimals{6}\showpercentage \\
\adaedsr + \DA ($10\times$) + AugMix  & \textbf{7.83\%} & 8\showdecimals{8}\showpercentage & 7\showdecimals{8}\showpercentage & 11\showdecimals{2}\showpercentage & 5\showdecimals{9}\showpercentage & \textbf{10\showdecimals{7}\showpercentage} & \textbf{7\showdecimals{3}\showpercentage} & 6\showdecimals{5}\showpercentage & 8\showdecimals{5}\showpercentage & 6\showdecimals{7}\showpercentage & 8\showdecimals{7}\showpercentage & 5\showdecimals{2}\showpercentage & 6\showdecimals{2}\showpercentage & 8\showdecimals{5}\showpercentage & 7\showdecimals{7}\showpercentage & \textbf{7\showdecimals{8}\showpercentage} \\
\DA  & 11.67\% & 12\showdecimals{1}\showpercentage & 10\showdecimals{2}\showpercentage & 15\showdecimals{2}\showpercentage & 7\showdecimals{1}\showpercentage & 20\showdecimals{5}\showpercentage & 12\showdecimals{2}\showpercentage & 8\showdecimals{4}\showpercentage & 12\showdecimals{3}\showpercentage & 9\showdecimals{8}\showpercentage & 9\showdecimals{3}\showpercentage & 6\showdecimals{7}\showpercentage & 13\showdecimals{1}\showpercentage & 11\showdecimals{8}\showpercentage & 14\showdecimals{1}\showpercentage & 12\showdecimals{2}\showpercentage \\
\DA + AugMix  & 10.15\% & 10\showdecimals{9}\showpercentage & 9\showdecimals{4}\showpercentage & 10\showdecimals{8}\showpercentage & 7\showdecimals{0}\showpercentage & 18\showdecimals{2}\showpercentage & 10\showdecimals{4}\showpercentage & 7\showdecimals{7}\showpercentage & 10\showdecimals{6}\showpercentage & 8\showdecimals{7}\showpercentage & 9\showdecimals{3}\showpercentage & 6\showdecimals{3}\showpercentage & 8\showdecimals{6}\showpercentage & 11\showdecimals{4}\showpercentage & 12\showdecimals{3}\showpercentage & 10\showdecimals{7}\showpercentage \\
\DA ($10\times$)  & 8.30\% & 9\showdecimals{0}\showpercentage & \textbf{7\showdecimals{6}\showpercentage} & 11\showdecimals{5}\showpercentage & \textbf{5\showdecimals{4}\showpercentage} & 14\showdecimals{0}\showpercentage & 7\showdecimals{9}\showpercentage & \textbf{6\showdecimals{1}\showpercentage} & 8\showdecimals{6}\showpercentage & \textbf{6\showdecimals{6}\showpercentage} & 7\showdecimals{1}\showpercentage & 5\showdecimals{0}\showpercentage & 7\showdecimals{3}\showpercentage & 9\showdecimals{1}\showpercentage & 10\showdecimals{0}\showpercentage & 9\showdecimals{4}\showpercentage \\
\DA ($10\times$) + AugMix  & 8.11\% & \textbf{8\showdecimals{8}\showpercentage} & 7\showdecimals{7}\showpercentage & \textbf{8\showdecimals{6}\showpercentage} & 5\showdecimals{7}\showpercentage & 14\showdecimals{4}\showpercentage & 7\showdecimals{9}\showpercentage & 6\showdecimals{2}\showpercentage & 8\showdecimals{4}\showpercentage & 6\showdecimals{7}\showpercentage & 7\showdecimals{3}\showpercentage & 5\showdecimals{1}\showpercentage & 6\showdecimals{5}\showpercentage & 9\showdecimals{2}\showpercentage & 10\showdecimals{4}\showpercentage & 8\showdecimals{9}\showpercentage \\
AugMix  & 13.13\% & 26\showdecimals{2}\showpercentage & 18\showdecimals{3}\showpercentage & 10\showdecimals{6}\showpercentage & 7\showdecimals{2}\showpercentage & 32\showdecimals{8}\showpercentage & 10\showdecimals{4}\showpercentage & 9\showdecimals{0}\showpercentage & 10\showdecimals{5}\showpercentage & 10\showdecimals{1}\showpercentage & \textbf{6\showdecimals{3}\showpercentage} & 4\showdecimals{7}\showpercentage & 6\showdecimals{3}\showpercentage & 11\showdecimals{4}\showpercentage & 20\showdecimals{1}\showpercentage & 13\showdecimals{0}\showpercentage \\
Nominal  & 25.17\% & 58\showdecimals{3}\showpercentage & 44\showdecimals{6}\showpercentage & 49\showdecimals{1}\showpercentage & 15\showdecimals{4}\showpercentage & 44\showdecimals{7}\showpercentage & 19\showdecimals{7}\showpercentage & 19\showdecimals{4}\showpercentage & 15\showdecimals{6}\showpercentage & 17\showdecimals{9}\showpercentage & 10\showdecimals{0}\showpercentage & 5\showdecimals{5}\showpercentage & 17\showdecimals{2}\showpercentage & 15\showdecimals{3}\showpercentage & 24\showdecimals{7}\showpercentage & 19\showdecimals{8}\showpercentage \Bstrut \\
\hline
\end{tabular}
}
\end{center}

==> tables/mce_imagenet.tex <==
\begin{center}
\resizebox{0.92\textwidth}{!}{
\begin{tabular}{l|c|ccc|cccc|cccc|cccc}
    \hline
    \cellcolor{header} & \cellcolor{header} & \multicolumn{3}{c|}{\cellcolor{header} \textsc{Noise}} & \multicolumn{4}{c|}{\cellcolor{header} \textsc{Blur}} & \multicolumn{4}{c|}{\cellcolor{header} \textsc{Weather}} & \multicolumn{4}{c}{\cellcolor{header} \textsc{Digital}} \Tstrut \\ 
    \cellcolor{header} \textsc{Setup} & \cellcolor{header} \textsc{mCE} & \cellcolor{header} \rotcol{Gauss} & \cellcolor{header} \rotcol{Shot} & \cellcolor{header} \rotcol{Impulse} & \cellcolor{header} \rotcol{Defocus} & \cellcolor{header} \rotcol{Glass} & \cellcolor{header} \rotcol{Motion} & \cellcolor{header} \rotcol{Zoom} & \cellcolor{header} \rotcol{Snow} & \cellcolor{header} \rotcol{Frost} &  \cellcolor{header} \rotcol{Fog} & \cellcolor{header} \rotcol{Bright} & \cellcolor{header} \rotcol{Contrast} & \cellcolor{header} \rotcol{Elastic} & \cellcolor{header} \rotcol{Pixel} & \cellcolor{header} \rotcol{JPEG} \Bstrut \\
    \hline    
\adaedsrcae + \DA + AugMix  & \textbf{67.36\%} & \textbf{48\showdecimals{3}\showpercentage} & \textbf{48\showdecimals{1}\showpercentage} & \textbf{48\showdecimals{9}\showpercentage} & 62\showdecimals{7}\showpercentage & 65\showdecimals{7}\showpercentage & 60\showdecimals{9}\showpercentage & 63\showdecimals{0}\showpercentage & 55\showdecimals{9}\showpercentage & \textbf{52\showdecimals{0}\showpercentage} & 44\showdecimals{0}\showpercentage & 36\showdecimals{4}\showpercentage & 44\showdecimals{1}\showpercentage & 56\showdecimals{0}\showpercentage & \textbf{56\showdecimals{8}\showpercentage} & 44\showdecimals{8}\showpercentage \Tstrut \\
\adaedsrcae + AugMix  & 72.23\% & 61\showdecimals{6}\showpercentage & 61\showdecimals{1}\showpercentage & 64\showdecimals{7}\showpercentage & 66\showdecimals{0}\showpercentage & 69\showdecimals{0}\showpercentage & 60\showdecimals{3}\showpercentage & 60\showdecimals{8}\showpercentage & 58\showdecimals{0}\showpercentage & 55\showdecimals{6}\showpercentage & 41\showdecimals{2}\showpercentage & 33\showdecimals{4}\showpercentage & \textbf{41\showdecimals{1}\showpercentage} & 54\showdecimals{0}\showpercentage & 60\showdecimals{3}\showpercentage & 60\showdecimals{2}\showpercentage \\
\adaedsr + AugMix  & 73.59\% & 67\showdecimals{3}\showpercentage & 68\showdecimals{2}\showpercentage & 71\showdecimals{7}\showpercentage & 65\showdecimals{6}\showpercentage & 73\showdecimals{8}\showpercentage & 62\showdecimals{8}\showpercentage & 61\showdecimals{1}\showpercentage & 61\showdecimals{3}\showpercentage & 58\showdecimals{7}\showpercentage & 39\showdecimals{6}\showpercentage & \textbf{31\showdecimals{9}\showpercentage} & 43\showdecimals{2}\showpercentage & 55\showdecimals{6}\showpercentage & 60\showdecimals{8}\showpercentage & 48\showdecimals{5}\showpercentage \\
\adacae + AugMix  & 80.85\% & 87\showdecimals{4}\showpercentage & 86\showdecimals{6}\showpercentage & 91\showdecimals{2}\showpercentage & 66\showdecimals{7}\showpercentage & \textbf{65\showdecimals{7}\showpercentage} & 63\showdecimals{0}\showpercentage & 63\showdecimals{0}\showpercentage & 71\showdecimals{3}\showpercentage & 66\showdecimals{0}\showpercentage & 50\showdecimals{6}\showpercentage & 42\showdecimals{2}\showpercentage & 52\showdecimals{2}\showpercentage & \textbf{53\showdecimals{5}\showpercentage} & 59\showdecimals{1}\showpercentage & \textbf{44\showdecimals{6}\showpercentage} \\
\DA  & 73.04\% & 52\showdecimals{1}\showpercentage & 52\showdecimals{1}\showpercentage & 53\showdecimals{3}\showpercentage & 60\showdecimals{5}\showpercentage & 69\showdecimals{0}\showpercentage & 65\showdecimals{9}\showpercentage & 63\showdecimals{3}\showpercentage & 57\showdecimals{7}\showpercentage & 55\showdecimals{4}\showpercentage & 43\showdecimals{8}\showpercentage & 33\showdecimals{8}\showpercentage & 58\showdecimals{2}\showpercentage & 56\showdecimals{2}\showpercentage & 66\showdecimals{8}\showpercentage & 63\showdecimals{8}\showpercentage \\
\DA + AugMix  & 70.05\% & 50\showdecimals{5}\showpercentage & 50\showdecimals{0}\showpercentage & 51\showdecimals{5}\showpercentage & \textbf{58\showdecimals{0}\showpercentage} & 67\showdecimals{8}\showpercentage & \textbf{60\showdecimals{1}\showpercentage} & \textbf{58\showdecimals{7}\showpercentage} & \textbf{54\showdecimals{5}\showpercentage} & 53\showdecimals{3}\showpercentage & \textbf{37\showdecimals{5}\showpercentage} & 33\showdecimals{4}\showpercentage & 43\showdecimals{6}\showpercentage & 56\showdecimals{8}\showpercentage & 64\showdecimals{2}\showpercentage & 72\showdecimals{0}\showpercentage \\
AugMix  & 77.12\% & 70\showdecimals{4}\showpercentage & 71\showdecimals{6}\showpercentage & 75\showdecimals{6}\showpercentage & 67\showdecimals{2}\showpercentage & 75\showdecimals{1}\showpercentage & 64\showdecimals{0}\showpercentage & 59\showdecimals{0}\showpercentage & 60\showdecimals{9}\showpercentage & 61\showdecimals{1}\showpercentage & 37\showdecimals{9}\showpercentage & 34\showdecimals{7}\showpercentage & 46\showdecimals{9}\showpercentage & 57\showdecimals{5}\showpercentage & 71\showdecimals{4}\showpercentage & 55\showdecimals{9}\showpercentage \\
Nominal  & 82.40\% & 73\showdecimals{2}\showpercentage & 74\showdecimals{8}\showpercentage & 80\showdecimals{1}\showpercentage & 71\showdecimals{4}\showpercentage & 78\showdecimals{5}\showpercentage & 70\showdecimals{4}\showpercentage & 65\showdecimals{4}\showpercentage & 66\showdecimals{7}\showpercentage & 63\showdecimals{6}\showpercentage & 46\showdecimals{1}\showpercentage & 35\showdecimals{8}\showpercentage & 63\showdecimals{3}\showpercentage & 57\showdecimals{4}\showpercentage & 72\showdecimals{4}\showpercentage & 55\showdecimals{9}\showpercentage \Bstrut \\
\hline
\end{tabular}
}
\end{center}
